The Multi-BMBY Mechanism: Proportionality-Preserving and Strategyproof Ownership Restructuring in Private Companies

In privately held startups, restructuring ownership is challenging due to diverse and uncertain valuations among owners. Traditional approaches, including the BMBY mechanism for equal partnerships, fail to address the complexities of multi-owner settings and don't elicit true valuations. We propose a novel mechanism that extends the BMBY rationale to accommodate these complex scenarios. Our mechanism ensures truthful valuation elicitation while offering several advantages: it is easy to implement, budget balanced, resistant to collusion, individually rational, and allocates shares to those who value them most. Crucially, it preserves proportionality among remaining owners, maintaining existing power dynamics. The mechanism allows for adaptive control of the eventual number of owners, addressing unique startup needs such as incentivizing employee ownership. This paper contributes to the field of ownership restructuring by providing a practical, theoretically-grounded solution for the complex dynamics of startup recapitalization, potentially improving decision-making processes and stakeholder relationships in these pivotal business transitions.

==> conc.tex <==
Testing one two three

==> intro.tex <==
Firms often need to perform ownership restructure. This may be due to a major strategic shift, just before a merger or an acquisition, or simply due to co-owners' desire to dissolve their partnership.  If the firm is public, it can trigger a ``share buyback'' process in which it absorbs the shares of interested sellers at the market price. Such buybacks have gained popularity since the 1980s, and are often considered a good omen as to the firm's financial fortitude (\citealp{Wohlner2019}). 
	
	The "buyback" mechanism in public firms exists due to the availability of a market price which serves as an anchor to the seller compensation. This anchor price does not exist in privately held firms which constitute the vast majority of companies in the US (e.g., in 2013, less than 15\% of the firms with over 500 employees were public and in 2010 private firms account for 59\% of US sales, \citealp{Biery2019}). For this sector, which comprises various firm sizes ranging from small mom-and-pop shops to huge conglomerates (\citealp{Forbes2019}), the buyback mechanism cannot simply be applied and often requires a costly due diligence process to assess the company share value.  
	
	When the firm is co-owned by two partners, each owning half, there exists an alternative ownership restructuring mechanism called "BMBY - buy me out or I will buy you out". The BMBY mechanism works as follows, say Alice and Bob co-own an indivisible asset, and wish to part ways. In BMBY, one partner, say Alice, declares a price and the other partner, Bob, decides whether he wants to buy Alice out or sell his share to Alice at the aforementioned price. This simple mechanism is extremely useful and intuitive, yet may be susceptible to strategic behavior and may lead to an inefficient allocation.\footnote{To see why, assume that agent types are determined by i.i.d draws from a uniform distribution over $[0,1],$ and consider a case where Alice's valuation is extremely low. In this case, as Bob's expected value is half, she can benefit from misreporting her value and declaring a higher price.
		%.... for any price declared by Alice, Bob will buy whenever $v_B\ge p$ and sell otherwise. Alice, who knows this will therefore bid $p=\frac{1}{2}v_A+\frac{1}{4},$ which unless $v_A=0.5$, does not equal her value.
	}
	
	
	In this work we extend the simple two agent BMBY mechanism to a setting in which the asset is owned by many share holders, while maintaining the mechanism simplicity.  We introduce a mechanism for decreasing the number of owners of a stock from $n$ to at most $\bar{m}<n$ (where $\bar{m}$ is exogenous), which we call Multi-BMBY Mechanism (MBM). The mechanism receives bids from all agents, and sets an asset price, at which agents trade shares of the asset. The eventual number of owners $m$ is a random variable that can be either $\bar{m}$ or $\bar{m}-1$, with a carefully chosen probability. 
 The mechanism is strategyproof: for each agent either increasing or decreasing her truthful bid does not increase her gain, regardless of the bidding of other agents. Additionally, the mechanism is immune to collusions (weak group strategyproof), budget balanced, and individually rational.

Regarding efficiency, it is evident that the most effective allocation method is to assign the entire asset to the agent who values it the most. However, this first-best allocation cannot be achieved by any incentive-compatible and budget-balanced mechanism, even in the bilateral trading case, as shown by the celebrated paper of \cite{myerson1983efficient}. While previous work has focused on developing such mechanisms that are \emph{approximately} efficient (\citealp{Reallocation-mechanisms,blumrosen2021almost}), our work considers the case in which a more distributed allocation is desired due to \emph{normative} reasons, such as safeguarding the rights of minority shareholders or preserving employees' stakes in ownership. 

We therefore introduce a mechanism that receives $\bar{m}$ as an input, and outputs an allocation in which the proportionality of the remaining ($\bar{m}$ or $\bar{m}-1$) owners' shares is preserved with respect to their initial shares. If an allocation satisfies this condition and allocates the asset to the set of agents with the highest valuations, we say that the allocation satisfies \emph{proportionally-preserving ex-post efficiency}. Our proposed mechanism indeed satisfies this property.

\subsection{Motivation}

Our approach differs from traditional ownership restructuring methods in two fundamental ways. First, instead of aiming for complete dissolution, we allow the final number of owners to be determined exogenously (up to one shareholder, in order to maintain strategyproofness). Second, we ensure that the allocation preserves the proportional shares of the original allocation. These constraints, while prioritizing proportionality and adaptability, may come at the cost of overall social welfare—typically the main focus of standard approaches for restructuring mechanisms. Imposing those axioms reflects some level of mismatch between the agents' welfare and the designer's objective.
One practical scenario where this approach is particularly relevant is during the restructuring of ownership in a privately held startup company before a potential acquisition. 

In the dynamic world of privately held startups, ownership structures often become complex and misaligned over time. Consider a technology startup that has pivoted several times since its inception. Over the years, it has accumulated a diverse array of owners—early investors, venture capital firms, angel investors, and former employees who received equity compensation. While this broad ownership base was crucial for the company's growth, it now presents challenges as the company enters a new strategic phase (e.g., prepares for a potential acquisition or pivot). The current owners wish to streamline the cap table, reducing the number of shareholders to simplify negotiations and decision-making processes. However, they face a delicate balancing act: they need to preserve the existing power dynamics among the remaining owners while ensuring that those who value the company most retain their stakes.
Furthermore, maintaining a significant number of owners post-restructuring is vital, as ownership tends to enhance job quality and boost employee commitment (see e.g. \citealp{gornall2024employees}).
Traditional methods fall short in addressing these competing objectives simultaneously. 

Share buybacks, a common approach for public companies, face a fundamental challenge in private firms: the lack of a predetermined market price. This absence makes it difficult to set a fair buyback price that reflects the true value of the company and accounts for the differing valuations of diverse owners. Sequential negotiations can be time-consuming, prone to strategic manipulation, and may not result in an efficient allocation. Both methods struggle to preserve proportionality among remaining owners while ensuring that those with the highest valuations retain their stakes. This scenario illustrates a common challenge in ownership restructuring of privately held assets—how to efficiently reallocate shares while maintaining proportionality among remaining owners and maximizing overall welfare, all without the benefit of a market-determined price. In this paper, we present a novel mechanism that tackles these challenges head-on.

% One practical scenario where our approach is particularly relevant is during the restructuring of ownership in a privately held startup company before a potential acquisition. In such cases, the company may wish to reduce the number of owners while ensuring that a certain level of employee ownership is maintained. This helps preserve the employees' stakes and their incentives to contribute to the company's success. Moreover, it is crucial to maintain the proportionality of the remaining shares to respect the initial ownership structure and to avoid any disruption in the perceived fairness among stakeholders. The proposed notion of proportionally-preserving ex-post efficiency balances those arguments with economic welfare. We also highlight that in such scenarios, the uncertainty regarding whether the final number of owners is $\bar{m}$ or $\bar{m}-1$ is insignificant, as long as the other desirable economic properties hold.
	
	

==> model.tex <==
Let $I = \{1, ..., n\}$ be the set of agents such that $n > 2$. For any subset of agents $J \subseteq I$, we denote by $|J|$ the number of agents in $J$. Each agent $i \in I$ has a private value $v_i \in \mathbb{R_+}$ for the asset.
	% The private values can be completely arbitrary and we do not assume that they are drawn from any particular distribution.
	Let allocation space $\mathcal{A} \subset \Delta^n \times \mathbb{R}^n$ consist of allocations for shares and money for all $n$ agents, where $\Delta^n$ is the $n-$dimensional simplex.
	Denote respectively by $s_i^A, x_i^A$ the share and money of agent $i$ under allocation $A$. 
	
	
	The MBM is a mapping $F: \mathcal{A} \times \mathbb{R}^n \rightarrow \mathcal{A}$ from an initial allocation and a bid vector to a new allocation. For each agent $i$, the mechanism defines the agent's monetary payment, which can be positive or negative, and resulting share, which is non-negative. 
	
	Denote by $u_i (s_i, x_i) = s_i v_i + x_i$ the utility of agent $i$  from shares $s_i$, and money $x_i$. We normalize the initial amounts of money to be zero, and therefore the initial utility of each agent is simply $s_i v_i$. In addition, we assume agents face no monetary constraints.
	The planner employs the mechanism to reallocate shares and money among the owners in a way that a subset $M \subset I$ of the initial owners remain owners at the end of the process. 
	
	For the reallocation process, the mechanism receives declarations from all $n$ agents of their valuation of the asset as bids $(b_i)_{i \in I}$  and selects $1 \le m < n$ agents who remain owners.  The other $n-m$ initial owners sell their holdings. 
	The mechanism also decides on a single asset price $p$ that is used for all sales and purchases of shares.
	Denote by $A_0$ the initial allocation and by $(\bar{b}_{i})_{i \in I} = (v_{i})_{i \in I}$ and $\bar{A} = F(A_0, (v_i)_{i \in I})$ the bids and allocation when all agents bid their private valuation.
	
	The mechanism works as follows: the planner limits the number of eventual owners with $\bar{m}$ that satisfies $1 < \bar{m} < n$.
 % \footnote{The case where the desirable outcome is the efficient allocation in which a single agent owns the entire asset can be solved by simply running a second-price auction while ignoring the initial shares. Our mechanism is designated for the case in which it is desirable to keep the asset distributed among multiple shareholders (and maintain proportionality with respect to the initial shares) for normative reasons.} 
 Each agent bids $b_i$ as a price for the whole asset, which represents her proportional declared valuation to every share size. Agents are ranked by their bids in \textbf{descending} order. We assume there are no ties in the agents' valuations.\footnote{Alternatively, one can assume that the agent valuations are drawn i.i.d. from an atom-less distribution and that ties occur with probability zero.} 
	 Let subscript $(i)$ denote the order statistic of bids such that $s^{A}_{(1)}$ is the share of the \textbf{highest} bidder. 
  Let $r((b_j)_{j \in I},i)$ denote the ranking of agent $i$ in $(b_j)_{j \in I}$ (i.e., agent $i$ for which $r(i)=1$ is the agents with the highest bid). When clear from context, we suppress $(b_j)_{j \in I}$ and write $r(i)$ for brevity.
	Then, the mechanism chooses the number of eventual owners $m\in\{\bar{m} - 1,\bar{m}\}$ at random (we describe the probabilities below), where $m = \bar{m}$ means that the $\bar{m}$'th ranked agent becomes a buyer, while $m = \bar{m} - 1$ means that the $\bar{m}$'th ranked agent becomes a seller. 
	
	We set the probability of $m = \bar{m}$ and $m = \bar{m} - 1$ in a way which makes the $m$'th ranked agent receive a utility of zero in expectation.  
	As we show later, the resulting probability for $m = \bar{m}$ is $\sum_{i=1}^{\bar{m}} s^{A_0}_{(i)}$ , (sum of the initial shares of the $\bar{m}$ highest bidders) and the probability for $m = \bar{m} - 1$ is $\sum_{i=\bar{m}+1}^{n} s^{A_0}_{(i)}$. 
	
	
	The mechanism then sets $p=b_{(\bar{m})},$ i.e., the price equals the $\bar{m}$'th highest ranked agent's bid. A higher bidder agent, say agent $j$, becomes a buyer. Her share in the final allocation increases by $s^{A_0}_{j}\frac{\sum_{i=m+1}^{n} s^{A_0}_{(i)}}{\sum_{i=1}^{m} s^{A_0}_{(i)}} > 0$ (i.e., by a factor of $\frac{1}{\sum_{i=1}^{m} s^{A_0}_{(i)}} > 1$), and all lower bidder agents become sellers to whom the mechanism allocates no shares. All low bidders receive compensation, which equals the price times their respective share in the initial allocation. 
	Denote by $\bar{r}, \bar{p}$ the ranking and price, respectively, when all agents bid their private valuation. %, and let $\bar{j}$ be the $\bar{m}$'th highest ranked agent in $\bar{r}$.
	
	%\begin{definition}
	%	For ranking $r$ and agent $j$ let $r_j$ be the partial ranking of agents ranked below $j$.
	%\end{definition}
	
	\subsection{Definitions}
	%\red{Gal: I'm not clear on whether you want to call this strategyproof or IC, so make the change if it's needed or talk to me about it}

    We begin by providing a formal definition of the MBM:

    \begin{definition}
        The Multi-BMBY Mechanism (MBM) $F$ receives as an input the initial allocation $A_0$ and a bidding profile $(b_i)_{i \in I} \in \mathbb{R}^n$, and outputs the following allocation:

        $$s_{(j)}^{F(A_0, (b_i)_{i \in I})} = \begin{cases}
        s_{(j)}^{A_0} \bigg( 1 + \frac{\sum_{i=m+1}^{n} s^{A_0}_{(i)}}{\sum_{i=1}^{m} s^{A_0}_{(i)}} \bigg)  & j \le m \\
        0 & j > m
        \end{cases} 
        % = \begin{cases}
        % \frac{s_{(j)}^{A_0}}{\sum_{i=1}^{m} s^{A_0}_{(i)}} & j \ge n - m + 1 \\
        % 0 & j < n - m + 1
        % \end{cases}
        $$

        $$x_{(j)}^{F(A_0, (b_i)_{i \in I})} = \begin{cases}
        -s_{(j)}^{A_0} \frac{\sum_{i=m+1}^{n} s^{A_0}_{(i)}}{\sum_{i=1}^{m} s^{A_0}_{(i)}} p  & j \le m \\
        s_{(j)}^{A_0} p & j > m
        \end{cases}$$

        where $p = b_{(\bar{m})}$ and $m=\bar{m}$ with probability $\sum_{i=1}^{\bar{m}} s^{A_0}_{(i)}$, and $m = \bar{m} - 1$ otherwise.
    \end{definition}
    
	Below we introduce the mechanism characteristics we wish to analyze. These properties are analogous to the properties studied by \cite{myerson1983efficient} in a bilateral trading framework.
    We start by defining the well-known notion of a ``strategyproof" mechanism. A mechanism is considered \textit{strategyproof} if bidding one's private value is a weakly dominant strategy for all agents, regardless of all the other agent bids. Formally:
	\begin{definition}
		A mechanism is considered \textit{strategyproof} if for every agent $i \in I$, every $(b_i)_{i \in I} \in \mathbb{R}^n$, and every $A_0 \in \mathcal{A}$, it holds that
		$$u_i(s^{F(A_0,(\bar{b}_i,b_{-i}))}_i, x^{F(A_0,(\bar{b}_i,b_{-i}))}_i) \geq u_i(s^{F(A_0,(b_i,b_{-i}))}_i, x^{F(A_0,(b_i,b_{-i}))}_i)$$
		where $b_{-i}$ are the bids of all the agents other than $i$.
	\end{definition}
	
	While the definition above tackles the case in which a single agent deviates, our mechanism also resolves cases in which a subset of agents all benefit from working in collusion. Next, we define the notion of a weak group strategyproof mechanism. A mechanism is considered \textit{weak group strategyproof} if it is impossible for all the agents who deviate from bidding their private valuation to strictly benefit simultaneously. Formally:
	
	\begin{definition}
		A mechanism is considered \textit{weak group strategyproof} if there does not exist a subset of agents $J \subseteq I$, bids $(b_i)_{i \in J} \in \mathbb{R}^{||J||}$, and initial allocation $A_0 \in \mathcal{A}$, such that for every agent $j \in J$, it holds that
		$$u_j\bigg(s^{F(A_0,((b_i)_{i \in J},(\bar{b}_i)_{i \in I \setminus J}))}_j, x^{F(A_0,((b_i)_{i \in J},(\bar{b}_i)_{i \in I \setminus J}))}_j\bigg) > u_j(s^{\bar{A}}_j, x^{\bar{A}}_j)$$
	\end{definition}
	
	Next, we define the notion of a budget balanced mechanism. Note that our definition of budget balanced, also includes a requirement that the asset will be fully allocated.
	\begin{definition}
		We say that a mechanism $F$ is \textit{budget balanced} if for every $(b_i)_{i \in I} \in \mathbb{R}^n$, and every $A_0 \in \mathcal{A}$, it holds that
		$$\sum_{i \in I} s^{F(A_0,(b_i)_{i \in I})}_i = \sum_{i \in I} s^{A_o}_i$$
		and
		$$\sum_{i \in I} x^{F(A_0,(b_i)_{i \in I})}_i = \sum_{i \in I} x^{A_o}_i$$
	\end{definition}
	
	
        When considering a strategyproof mechanism, it is sufficient to discuss the outcome of the mechanism in the case where agents play their dominant strategy, which is bidding their true valuations. Hence the following two properties, which are related to the quality of the outcome, are only defined with respect to truthful bidding of the agents.
        
         While it is clear that efficiency can only be obtained by allocation of the asset to the agent with the highest valuation, many real-life applications require distributing the asset among a larger, predefined number of agents. A natural weaker requirement of such distribution is that the asset is allocated to the set agents who value it the most. While there are infinitely many such allocations, a second natural requirement is that the allocation preserves the proportional share of each agent compared to the initial allocation. That is, an allocation $A$ is said to be proportionality-preserving with respect to initial allocation $A_0$ if for every pair of owners in $A$, the ratio between their eventual shares is the same as the share between their initial shares. \textit{Proportionality-preserving Ex-post efficiency} is then defined as follows:

        \begin{definition}
            We say that a mechanism $F$ satisfies \textit{proportionality-preserving ex-post efficiency} if for every $A_0 \in \mathcal{A}$, the allocation $\bar{A}$ satisfies the following two conditions:
            \begin{enumerate}
                \item For any two agents $j, k \in I$ such that $s_j^{\bar{A}} > 0$ and $s_k^{\bar{A}} > 0$ (both agents are buyers), it holds that $\frac{s_j^{\bar{A}}}{s_k^{\bar{A}}} = \frac{s_j^{A_0}}{s_k^{A_0}}$.
                \item There exists no pair of agents $j, k \in I$ such that $s_j^{\bar{A}} = 0$ (agent $j$ is a seller), $s_k^{\bar{A}} > 0$ (agent  $k$ is a buyer), and $v_j > v_k$. 
            \end{enumerate}
        \end{definition}

        Finally, we define \textit{individual rationality}, which implies that under truthful bidding all agents improve their utility with respect to the initial allocation:
        
	\begin{definition}
		We say that a mechanism $F$ satisfies \textit{individual rationality} if for every $j\in I$ and every $A_0 \in \mathcal{A}$, it holds that
		$$u_j(s_j^{\bar{A}},x_j^{\bar{A}})\ge u_j(s_j^{A_0},x_j^{A_0})$$
	\end{definition}
	
	Lastly, we define the useful notion of \textit{adjusted utility}, which is simply the difference between the agent's utility before and after applying a restructuring mechanism:
 \begin{definition}
     Given an allocation $A \in \mathcal{A}$, the \textit{adjusted utility} of agent $j$ with respect to the initial allocation $A_0 \in \mathcal{A}$ is defined as follows:
     $$\tilde{u}_j(s_j^{A},x_j^{A}) = u_j(s_j^{A},x_j^{A}) - u_j(s_j^{A_0},x_j^{A_0})$$
 \end{definition}

 Note that individual rationality can be redefined by requiring that the adjusted utility of each agent with respect to the allocation obtained by truthful bidding is non-negative. Moreover, note that since the initial utilities are constant, properties like strategyproof and weak group strategyproof can be equivalently defined with respect to the adjusted utility, as agents always have a beneficial deviation with respect to their standard utility if and only if they have a  beneficial deviation with respect their adjusted utility. Therefore, from now on we only consider the agents' adjusted utility, without explicitly specifying it.
	
	%\begin{definition}
	%	We call deterministic mechanism to a mechanism which generates a deterministic allocation of both money and shares. In other words, it outputs the same result every time it runs on the same input.
	%\end{definition}
	
	
	%\begin{definition}
	%	We call an asymptotically deterministic mechanism to a mechanism which generates deterministic quantities of both money and shares to a ratio of agents that approaches $1$ when a number of agents goes to infinity.
	%\end{definition}
	

==> rel_lit.tex <==
Testing one two three
